Hybrid Aerial-Ground Vehicle Autonomy in GPS-denied Environments

The DARPA Subterranean Challenge is leading the development of robots capable of mapping underground mines and tunnels up to 8km in length and identify objects and people. Developing these autonomous abilities paves the way for future planetary cave and surface exploration missions. The Co-STAR team, competing in this challenge, is developing a hybrid aerial-ground vehicle, known as the Rollocopter. The current design of this vehicle is a drone with wheels attached. This allows for the vehicle to roll, actuated by the propellers, and fly only when necessary, hence benefiting from the reduced power consumption of the ground mode and the enhanced mobility of the aerial mode. This thesis focuses on the development and increased robustness of the local planning architecture for the Rollocopter. The first development of thesis is a local planner capable of collision avoidance. The local planning node provides the basic functionality required for the vehicle to navigate autonomously. The next stage was augmenting this with the ability to plan more reliably without localisation. This was then integrated with a hybrid mobility mode capable of rolling and flying to exploit power and mobility benefits of the respective configurations. A traversability analysis algorithm as well as determining the terrain that the vehicle is able to traverse is in the late stages of development for informing the decisions of the hybrid planner. A simulator was developed to test the planning algorithms and improve the robustness of the vehicle to different environments. The results presented in this thesis are related to the mobility of the rollocopter and the range of environments that the vehicle is capable of traversing. Videos are included in which the vehicle successfully navigates through dust-ridden tunnels, horizontal mazes, and areas with rough terrain.

==> Chapters/00ProgressReport.tex <==
\chapter{Progress Report}
This section details the progress that has been made on the thesis to date. The first few weeks were spent familiarising with the project and the current code base. A local planner capable of generating polynomial-based trajectories and checking these paths for collisions with sample simulated obstacles had been created by another member of the team.

\section{Collision Avoidance}
The first step was to integrate information from real sensors into this package. An Intel RealSense camera was connected to the local planner code base on the computer and integrated with the collision checker. In addition, a method for visualising the results proved to be a necessity for debugging and was therefore developed in RViz. The visualisation shown in \ref{fig:prog_report} was created.\\

\begin{figure}[H]
	\centering
	\includegraphics[width=0.5\textwidth]{Figures/ProgressReport/collision_avoidance.png}
	\caption{Collision avoidance visualisation in RViz}
	\label{fig:prog_report}
\end{figure}

The coloured points represent the point cloud coming into the local planner. The lines forming a star at the origin are the motion primitives being considered. If the primitive is red, it indicates that there is a collision along that path. In this case, it was set to be considered as a collision if there was an obstacle within 30cm of the path.\\

There were many steps involved in integrating real data and visualising the results. First, the cloud needed to be processed. The following setup was made. First, the cloud is down-sampled from around 100,000 points to 2000 points, increasing the speed of the calculations. This is completed by creating a Voxel (volume-pixel) grid. If a grid point of a specified size has at  least a specified minimum number of points, a voxel is placed there. By tuning the size of the grid and the minimum number of points per voxel, one can ensure that outliers are not included and adjust the grid to a more usable number of points with the same filter. This filter also removes all the points at the origin (the location of the camera) and invalid points represented by ‘NaN’ (not a number).\\

The next stage of the cloud processing involves transforming the cloud to match the world. The points are extracted in the coordinate system of the camera (herein referred to as the camera frame) and need to be converted to the world coordinate system (the world frame). The world frame is determined using a simultaneous localisation and mapping (SLAM) algorithm. Our system uses orbSLAM. This algorithm provides the orientation in the same coordinate system based on the initial orientation of the camera, but with a different axis layout. This orientation provides the information required to create an Affine transformation matrix to transform the point cloud from the camera frame to the orbSLAM frame which, in the early stages of development, was considered to be the same as the world frame. Once this was implemented, rotating the camera led to the point cloud moving around the origin while the features would remain stationary. \\

Once the cloud had been processed, a KD-tree was generated for it such that the primitives could use a knn-search (‘k’ nearest neighbours search) to find the obstacles closest to the sample points along the primitives. The collision status of the primitive (whether or not it collides with any obstacles) was then correlated to a cost function. This allowed the points representing the primitives to be sent as type ‘PointXYZI’, meaning a location coordinate and an intensity, depicting the cost. A point with a higher cost (1, colliding) would be shown as red in RViz while a point with a lower cost (0, not colliding) would be shown in blue. \\

Once collision avoidance was fully functional and debugged on the computer with the camera connected, the code was transferred to the rollocopter. The rollocopter computer board is an Intel NUC which is effectively a very powerful computer which runs Ubuntu 16.04. Hence, the main task in this was to integrate the sensor with the on board inertial measurement unit (IMU). This is based on the same frame as gravity. An extended Kalman filter (EKF) had been created which can fuse the IMU data with the orbSLAM data. The resulting information was then used to transform the point cloud from the camera frame to the orbSLAM frame, then to the IMU frame, and finally to the world frame. \\% VIDEO LINK HERE??

Once the local planner node was capable of generating commands based on the sensory information from the sensors on the vehicle, it was integrated with the controller. At the moment, the controller is based on a pure pursuit model. While this is not using the trajectories effectively, it has been empirically shown to work effectively in most cases. With a deadline for the project in less than a month, the focus is on making this method more robust for a variety of cases. Once this demonstration is complete, the focus will be on methods which are more sophisticated.\\

A few improvements have been made to the collision avoidance system to make it more robust.
\begin{itemize}
\item \textit{Accounting for the field of view}\\
\indent As shown in Figure \ref{fig:prog_report}, there were primitives in all directions despite only having information within the 90$^o$ field of view of the camera. Hence, the primitives are now only generated within the field of view of the camera. In addition, when tested on the vehicle, it was found that there was some jittering when a primitive on the edge of the field of view was selected. This occurs when there was an obstacle near the edge of that primitive. When the vehicle chose the primitive, it would yaw towards it and see the obstacle, hence choosing another path. When it would yaw to the new path, it would then no longer see the previous obstacle and hence choose the primitive on the edge again. This back and forth is what caused the jittering. Thus, the primitives are now created within a slightly smaller angle range than the field of view.
\item \textit{Warping Transformation}\\
\indent Another issue was discovered where the ceiling would appear to warp in the visualisation when the vehicle rolled or pitched. This was fixed by saving the state at the time the cloud was received to ensure that the cloud was transformed by the corresponding state instead of the current state, after the cloud had been processed (downsampling and removing invalid points).
\item \textit{Ground interference}\\
\indent Given that the robot rolls, the ground is often in the field of view and is therefore included in the point cloud. This had to be filtered out when checking for collisions. The collision buffer was less than the distance between the camera and the ground leading to the primitives colliding when the ground portion of the point cloud was included.
\item \textit{Additional option when all primitives are colliding}\\
\indent When all the primitives collide, there is now a behaviour which causes a yawing motion. This leads to the field of view changing, leading to non-colliding paths becoming visible.
\end{itemize}

An image of the latest state is shown in Figure \ref{fig:CA_latest_pr}.

\begin{figure}[H]
	\centering
	\includegraphics[width=0.5\textwidth]{Figures/ProgressReport/collision_avoidance2.png}
	\caption{New collision avoidance shown in RViz}
	\label{fig:CA_latest_pr}
\end{figure}

\section{Wall Following}
The other main part of the project has been based on designing a system which can work without localisation. This was created from scratch and is currently capable of generating a wall-following path based on the current sensory information in the form of a point cloud. At first, this was set up as a simple algorithm in matlab which takes a planar wall, the normal of which is known, and converts the wall to a straight line in the body frame in 2D space. A second line, parallel to the wall line, is then defined based on a buffer distance of 30cm, for instance, which becomes the path for the rollocopter to follow.\\

This algorithm was then converted to C++ and implemented with the RealSense camera connected to the computer. An extra step for this is to extract the wall plane from the real data. The point cloud library (PCL) has a set of functions which use a random sample consensus (RANSAC) method for fitting shapes to the cloud. The plane fitting function was used on the point cloud to define the wall. A visualisation similar to the previous was then developed to show the velocity commands being sent to the controller with respect to the wall.\\

It was found that this works well for straight walls when the majority of the field of view of the camera is facing the wall. However, if the camera direction was mostly parallel to the wall (defined as a vector pointing straight out of the camera), then the RANSAC algorithm started to fit planes to the floor and the ceiling. To ensure this would not occur, a pass through filter was implemented such that the RANSAC algorithm would be used on a cloud that contained only points within the range in which wall is expected to appear. This involved limiting the z coordinate to above the ground and below the ceiling and keeping only the points with the same y coordinate sign to ensure that the wall on the other side was not being considered too. Once this had been implemented, the path line, and hence velocity commands, stopped changing so rapidly allowing the trajectory to be significantly smoother.

While testing the collision avoidance system, it was found that the walls are also treated as obstacles. As a result, the collision checking algorithm is capable of following the wall. Hence, the goal is set to be at a constant position of directly ahead in the body frame. This leads to the vehicle moving forward while avoiding collisions, thus following the wall. A video of this behaviour can be found \color{blue}\href{https://youtu.be/g23erB4Tx9g}{here}\color{white}.

\newpage
\section{Current and Future Work}
I am currently working on implementing a traversability analysis algorithm. When testing in a realistic environment, it was discovered that the vehicle experiences extreme instability when rolling over patches with rocks. The traversability analysis will use point clouds from the RGBD camera and extract an elevation map. The variance of discretised units of the elevation map will be used to determine the roughness. The slope will also be determined. In addition, the vehicle will be tested traversing a variety of rocks to gain insight into the capability.\\

This information will be combined to create a traversability map which will work in a manner analogous to an occupancy grid. Each patch of the ground will be represented  in the grid as whether or not it is traversable. If there are no fully traversable paths available, the vehicle will fly.


==> Chapters/3TheRollocopter.tex <==
\chapter{The Rollocopter}
\section{Hardware Design}
An insight into the hardware system is required to design an effective planner and control system. The original rollocopter design was used for the majority of the thesis. However, there was continued development on the hardware system while this thesis was in progress. Hence, the rollocopter hardware system at the end of the thesis is also described in this section.

\subsection{The Original Rollocopter}
The rollocopter was initially designed to be a drone with wheels such that the propellers would be the thrust force in both the aerial and ground mobility modes. The main advantage was that the vehicle would use less power when rolling than flying due to the thrust only being required to change the direction of the vehicle as opposed to keeping the vehicle at a constant height as well.
\begin{figure}[H]
	\centering
	\includegraphics[width=0.55\textwidth]{Figures/TheRollocopter/rollo_hw_1.png}
	\caption{Initial rollocopter design}
	\label{fig:initial_rollo_hw}
\end{figure}

\subsection{The Current Design}
\begin{figure}[H]
	\centering
%	\includegraphics[width=0.5\textwidth]{Figures/TheRollocopter/rollo_hw_2.png}
	\caption{Final rollocopter design}
	\label{fig:final_rollo_hw}
\end{figure}

\newpage
\section{Perception}
The perception subsystem has access to the following sensors. 
\begin{itemize}
	\item RealSense RGBD Camera
	\item Velodyne 360$^o$ LIDAR
	\item LIDAR-based height sensor
	\item Optical flow sensor
	\item Inertial Measurement Unit (IMU)
\end{itemize}

The solutions for localisation are still in development. However, there are multiple solutions which are currently being pursued. Visual-Inertial Odometry (VIO) is being used on the colour-based images from the RGBD camera. \color{red} DETAILS ABOUT HOW THIS WORKS AND HOW IT IS GOING\color{default}.

Another solution which is being considered is LIDAR-Inertial Odometry (LIO) which uses a SLAM algorithm known as LOAM on the LIDAR information from the Velodyne LIDAR. The Velodyne LIDAR is also used for the local maps and collision avoidance in the guidance and control system.
 
The LIDAR-based height sensor is considered to be a reliable method for obtaining an estimate of the height of the vehicle with respect to the ground and is used as the feedback for the controller. 
\newpage
\section{Autonomy and Control System}
The autonomy system is structured as shown in Figure \ref{fig:autonomy_system_architecture}.

\begin{figure}[H]
	\centering
	\includegraphics[width=0.5\textwidth]{Figures/TheRollocopter/SystemArchitecture.png}
	\caption{Autonomy system architecture}
	\label{fig:autonomy_system_architecture}
\end{figure}

\noindent\textbf{BPMN: Autonomy State Machine}\\
The 'Business Process Management' (BPMN) node is a system that works like a state machine. Given the current state and task of the system, the BPMN calculates the next desired behaviour of the system. This system is set up such that the following behaviours are possible.
\begin{itemize}
	\item List behaviours here...
	\item Wall following
	\item Continue to goal
	\item Return to base station
\end{itemize}

These behaviours are then sent to the Mobility Services node.

\noindent\textbf{Mobility Services}\\
Mobility Services uses the behaviour sent from the BPMN to determine the goals for the vehicle and sends these goals to the mid-level planner.

The behaviours are converted into services such as 'Take off', 'Land', 'Fly forward' and others, detailed in Chapter \ref{sec:MobilityServices}. The services are translated into a series of goals which can be sent to the mid-level planner. The resolution of these goals is of the order of 10s of metres.

\noindent\textbf{Local Mapper}\\
The local mapper creates a sub-map based on the point cloud from the LIDAR. The latest state estimate is used to transform the latest cloud into the map frame. The new cloud is then combined with the previous clouds from within a given radius of the current position. Octomap is used to create a map of the environment with occupied and unoccupied cells, as shown in Figure \ref{fig:local_map}.

\begin{figure}
	\centering
%	\includegraphics[width=0.5\textwidth]{Figures/TheRollocopter/local_map.png}
	\caption{Example of the local map}
	\label{fig:local_map}
\end{figure}

\noindent\textbf{Mid-level Planner}\\
The mid-level planner uses A* to plan an optimal path from the latest position of the vehicle to the goal from mobility services, based on the information in the local map. The planner then defines a waypoint which is 1m away from the vehicle, in the direction of the most optimal path.

\noindent\textbf{Local Planner}\\
The local planner receives the waypoint from the mid-level planner and generates a series of dynamically-feasible motion primitives from the current position. These primitives are discretised and checked for collisions. The primitive which is most towards the goal and collision free is then followed. The primitive is converted to a target velocity which can be sent to the controller.

\noindent\textbf{Controller}\\
The controller receives the velocity setpoint from the local planner and calculates the desired acceleration accordingly. This acceleration is converted into motor speeds in revolutions per minute (RPM) which is then sent to the PX4 flightstack. The flightstack is run on the Pixhawk which sends the commands to the motors.










%\section{Local System Architecture}
%This section details the architecture of the local planner and the adjacent nodes. 
%
%\begin{figure}[H]
%	\centering
%	\begin{subfigure}[b]{0.8\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{Figures/TheRollocopter/map_with_loc.png}
%		\caption{With Localisation}
%		\label{Rollocopter_map_with_loc}
%	\end{subfigure}
%	\vfill
%	\begin{subfigure}[b]{0.8\textwidth}
%		\centering
%		\includegraphics[width=\textwidth]{Figures/TheRollocopter/map_without_loc.png}
%		\caption{Without Localisation}
%		\label{Rollocopter_map_without_loc}
%	\end{subfigure}
%	\caption[Local Planner system architecture]{Map of inputs and outputs for the local planner node}
%	\label{subfig}
%\end{figure}
%
%
%In the figures above, the boxes represent nodes in ROS (robot operating system) and the arrows represent the messages being sent between the nodes. 
%
%
%In the case where localisation is accessible, the architecture in Figure \ref{Rollocopter_map_with_loc} is used. orbSLAM is an opensource SLAM algorithm which uses RGBD (red-green-blue-depth) data from the stereo camera or a point cloud from the LIDAR (Light Detection and Ranging device). The algorithm identifies features in the frames and uses the change in position of the features to calculate the change in the position of the camera. This allows for information about the position and orientation of the vehicle to be determined. Hence, the local planner is provided with a pose estimate 
%
%
%
%
%
%
%
%When localisation data is not reliable, the setup in Figure \ref{Rollocopter_map_without_loc} is implemented. The inertial measurement unit (IMU) is capable of sending reliable information about the pitch and roll of the vehicle. This allows for the point cloud to be transformed accordingly. Hence, when the wall following algorithm is running, the planner knows to ignore the floor and ceiling of the tunnel.


\section{Software Tools}
We used ros to communicate between the different systems on teh same 
wifi network. this will allow for us to do multi agent mapping. but 
first priority, which this project is geared toward, is getting a 
given vehicle to work well, before collaborating with others. 
focussing on the rollocopter. 
\subsection{ROS and Associated Tools}

% wROS[CITE_ROS]
 is a communications protocol which enables multiple 
nodes on the same wireless network to communicate. This allows for 
efficient and simple transference of information between different 
systems. For instance, the perception information from the sensors 
can be integrated with the ROS network using a ROS wrapper. 

For example, a planning node can then subscribe to the information 
from the sensors and publish commands which can be received by a 
controller.




==> Chapters/4CollisionAvoidanceAlgorithm.tex <==
\chapter{Collision Avoidance}\label{chap:LocalPlanner}
\section{Collision Avoidance Methods}
In this chapter, an approach for avoiding collisions in real time is presented. A requirement for this method is that it cause minimal latency, given that the planner cannot provide paths to the controller without this step being completed.

\section{Initial Setup}
The first step was to integrate information from real sensors into this package. An Intel RealSense camera was connected to the local planner code base on the computer and integrated with the collision checker. In addition, a method for visualising the results proved to be a necessity for debugging and was therefore developed in RViz. The visualisation shown in Figure 3.1 was created.

The coloured points represent the point cloud coming into the local planner. The lines forming a star at the origin are the motion primitives being considered. If the primitive is red, it indicates that there is a collision along that path. In this case, it was set to be considered as a collision if there was an obstacle within 30cm of the path.

There were many steps involved in integrating real data and visualising the results. First, the cloud needed to be processed. The following setup was made. First, the cloud is down-sampled from around 100,000 points to 2000 points, increasing the speed of the calculations. This is completed by creating a Voxel (volume-pixel) grid. If a grid point of a specified size has at least a specified minimum number of points, a voxel is placed there. By tuning the size of the grid and the minimum number of points per voxel, one can ensure that outliers are not included and adjust the grid to a more usable number of points with the same filter. This filter also removes all the points at the origin (the location of the camera) and invalid points represented by NaN (not a number).

The next stage of the cloud processing involves transforming the cloud to match the world. The points are extracted in the coordinate system of the camera (herein referred to as the camera frame) and need to be converted to the world coordinate system (the world frame). The world frame is determined using a simultaneous localisation and mapping (SLAM) algorithm. Our system uses orbSLAM. This algorithm provides the orientation in the same coordinate system based on the initial orientation of the camera, but with a different axis layout. This orientation provides the information required to create an Affine transformation matrix to transform the point cloud from the camera frame to the orbSLAM frame which, in the early stages of development, was considered to be the same as the world frame. Once this was implemented, rotating the camera led to the point cloud moving around the origin while the features would remain stationary.

Once the cloud had been processed, a KD-tree was generated for it such that the primitives could use a knn-search (k nearest neighbours search) to find the obstacles closest to the sample points along the primitives. The collision status of the primitive (whether or not it collides with any obstacles) was then correlated to a cost function. This allowed the points representing the primitives to be sent as type PointXYZI, meaning a location coordinate and an intensity, depicting the cost. A point with a higher cost (1, colliding) would be shown as red in RViz while a point with a lower cost (0, not colliding) would be shown in blue.

Once collision avoidance was fully functional and debugged on the computer with the camera connected, the code was transferred to the rollocopter. The rollocopter computer board is an Intel NUC which is effectively a very powerful computer which runs Ubuntu 16.04. Hence, the main task in this was to integrate the sensor with the on board inertial measurement unit (IMU). This is in a gravity-aligned frame. An extended Kalman filter (EKF) had been created which can fuse the IMU data with the orbSLAM data. The resulting information was then used to transform the point cloud from the camera frame to the orbSLAM frame, then to the IMU frame, and finally to the world frame.

Once the local planner node was capable of generating commands based on the sensory information from the sensors on the vehicle, it was integrated with the controller. At the point of testing this, the controller was based on a pure pursuit model. While this was not using the trajectories effectively, it had been empirically shown to work effectively in most cases.

\section{Issues from Hardware Tests and Improvements}
This method was tested in a variety of cases and the following issues were encountered and accounted for.

	\subsection{Field of view limitations}
	As shown in Figure 3.1, there were primitives in all directions despite only having information within the 90$^o$ field of view of the camera. Hence, the primitives are now only generated within the field of view of the camera. In addition, when tested on the vehicle, it was found that there was some jittering when a primitive on the edge of the field of view was selected. This occurs when there was an obstacle near the edge of that primitive. When the vehicle chose the primitive, it would yaw towards it and see the obstacle, hence choosing another path. When it would yaw to the new path, it would then no longer see the previous obstacle and hence choose the primitive on the edge again. This back and forth is what caused the jittering.
	
	The solution for this issue was to limit the primitives to be within the field of view of the camera. The given primitive considered to be free could then theoretically be reliably followed without risk of collision.
	 
	\subsection{Warping ceiling from previous transformation}
	Another issue was discovered where the ceiling would appear to warp when the vehicle rolled or pitched. This was fixed by saving the state at the time the cloud was received, instead of using the latest state when transforming. Accounting for this delay allowed for the transformations to be closer to the ground truth and therefore more usable.
	
	\subsection{Ground inteference}
	When the vehicle pitched forward, the ground was included in the field of view. Given that the collision buffer zone extended 2cm beyond the furthest edge of the wheels, the ground would appear to be in collision with the primitives. The solution to this was to truncate the cloud to occlude the ground region when the transform was accurate.
	
	\subsection{Additional option for when all primitives are stuck}
	An additional primitive was added outside the field of view such that when the main primitives were all in collision, the vehicle would have a tendency to yaw. This led to a different field of view, and therefore a higher chance of noticing possible primitives.

\section{Initial Results}
Show videos of these results and how it behaved, include video from B4 conference room test around box, discuss how it went, what it looked like, further developments
\section{Challenges Presented During Testing and Development}
\section{The Updated Cost Function}

\begin{figure}[H]
	\begin{subfigure}[b]{0.5\textwidth}
		\includegraphics[width=\linewidth]{Figures/CollisionAvoidance/collision_cost.png}
		\caption{Collision cost}
	\end{subfigure}
	\hfill
	\begin{subfigure}[b]{0.5\textwidth}
		\includegraphics[width=\linewidth]{Figures/CollisionAvoidance/goal_cost.png}
		\caption{Goal cost}
	\end{subfigure}
	\caption{Cost functions for primitives}
	\label{fig:cost_functions}
\end{figure}

\begin{figure}[H]
	\centering
	\includegraphics[width=0.5\textwidth]{Figures/CollisionAvoidance/total_cost.png}
	\caption{The resutling total cost}
	\label{fig:total_cost_function}
\end{figure}

\reddit{INSERT ALGORITHM WHICH DETAILS THE EQUATIONS OF THE COST AND THE RESULTING BEHAVIOUR}

\section{Improvements and Results}


==> Chapters/8LandingSiteDetection.tex <==
\chapter{Landing Site Detection}

==> Chapters/CaseStudy1_FlightMech.tex <==
\chapter{Case Study: Advanced Flight Mechanics}
This case study details how the material in the subject `Flight Mechanics Advanced Test and Evaluation' was covered in work relating to this thesis. The following lists the learning attributes as detailed in the handbook on the Course and Unit of Study Portal (CUSP).

\begin{itemize}
\item \textbf{Understanding of aircraft flight test, validation and verification}\\
describe how we did multiple rollo flight tests and used this to validate calculations for the controller

\item \textbf{Development of modern flight control, guidance, and navigation systems}\\
The rollocopter is a modern system which is still in development. The work in this thesis has been towards the Guidance and Control Team. As detailed in the respective sections of this report, this work has related to 
GNC - quick overview of everything we did, explain how it relates

\item \textbf{Aircraft System Identification and Control}\\
Describe controller work, tuning gains, weighing, and doing tests to measure the thrust rating 

\item \textbf{Autopilot Control Systems in Aircraft Operation}\\
Kind of covered 2 points above?? - but autonomous, not autopilot --> unmanned (all g?)

\item \textbf{Advanced Feedback Control Systems}\\
explain how we use the state estimation stuff in our control systems - essentially the closed loop diagram
(again...covered earlier in thesis)

\item \textbf{Concepts of Parameter and State Estimation and the Implementation of a Kalman Filter}\\
describe perception work - something about ekf2 from pixhawk and how this relates to the vehicle, any params we had to tune to get estimation to work - talk about params for lio stuff - gain tuning to remove effects of velodyne rotation on accelerometer causing unusual behaviour

\item \textbf{Multi-Loop Control and Guidance Systems and the Reasons for their Structures}\\
local mapper, local planner, controller - 3 loops at increasingly high frequency explain why structured like this.


\item\textbf{Flight Test Principles, Procedures and Implementation}\\
Pretty much just reiterate safety section from field tests and general flight testing.
\end{itemize}

==> Chapters/CaseStudy2_AircraftDesign.tex <==
\chapter{Case Study: Advanced Aircraft Design} \LARGE{\color{red} FIGURE OUT HOW TO RELATE THIS TO SUBT\color{default}}\normalsize
\begin{itemize}
 \item provide familiarity and understanding with practical aircraft design processes expected in industry


\item evaluation and case studies of existing aircraft designs. 


\item gain a better understanding of relevant issues particularly related to the design of aircraft with a level of confidence 


\item develop new designs or modifications, having a good balance between theory and real-world applications.


\item Good familiarity with unique and stringent international aviation regulations and certification processes will be expected with respect to the design of aircraft. 

\item aircraft specifications; 


\item aircraft selection and evaluation;


\item aircraft configuration design; 


\item design considerations for aerodynamics,


\item structures, systems, manufacture, 


\item testing, certification, life-cycle-cost, operations; 


\item the use of computational aircraft design tools, 


\item in particular DARcorp's Advanced Aircraft Analysis (AAA); and


\item introduction to multidisciplinary design optimisation methods.


\item Projects will be based on case study analyses and evaluation of aircraft types to operational specifications and requirements.

\end{itemize}


==> Chapters/OHS.tex <==
\chapter{Occupational Health and Safety}

\section{Safety Training}
Each worker is required to undertake the following safety courses.

\textbf{Personal Protective Equipment Overview:} Provided an overview of the equipment to use and when it should be used\\

\textbf{Eye and Face Protection: }This detailed the cases in which one is required to where glasses and masks. While testing the rollocopter, all observers are required to wear goggles. If the vehicle is connected to a handheld tether or is being used in a handheld test with the propellers being used, the person holding the tether is required to wear a face mask. \\ 

\textbf{Hand Protection:} This session covered which gloves should be worn during a range of circumstances. The relevant section for our team was that the person holding the tether or rollocopter must be wearing gloves.\\

\textbf{Robotic Safety:} This covered the importance of various aspects of safety protocols around robots. For instance, it is important to have emergency stop capabilities and designated testing areas that observers must not enter during tests.\\

\textbf{Electrical Safety: }The electrical safety course covered the required procedures for avoiding electrical fires. Notable points include not connecting multiple multi-adapters or extension cords in series ('daisy chains') and ensuring all wires are well insulated.\\

\textbf{Fire Extinguisher Training:} The fire department taught us which extinguishers need to be used in what circumstances and demonstrated how to use them. Practice runs were also included such that all workers could understand the required hand motion and how the fire extinguisher works.

\section{Testing Procedures}
JPL has strict testing requirements which must be adhered to. Depending on the nature of the testing, the requirements can differ, as detailed below.

\begin{itemize}
	\item Operating with a fixed tether
	\begin{itemize}
		\item The tether must be securely attached to a support surface, such as the ceiling
		\item Everyone in the vicinity of the test must wear glasses
		\item be ready to kill in case the propellers make contact with anything
		\item Stop the flight before the battery reaches 3.7V per cell
		\item In the case of a quadrotor, if its the first flight of the vehicle, hold the vehicle down (with gloves) and test that the response of the motors corresponds to the desired behaviour.
		\item Always have the tether attached to the vehicle and stay at least  the length of the tether away from vehicle
	\end{itemize}
	\item Operating with a moving tether
	\begin{itemize}
		\item In addition to the above requirements, the tether must be held with two hands and must follow the vehicle
	\end{itemize}
	\item Operating untethered (indoors only)
	\begin{itemize}
		\item In addition to the above requirements, the vehicle must be a testing area separated by a net.
		\item The pilot must stay away from vehicle, behind the net, if possible.
	\end{itemize}
	\item Autonomous flight\\
	In addition to the requirements above, if the vehicle is flown autonomously, one must also follow the guidelines below.
	\begin{itemize}
		\item Before commencing any test, ensure all of those involved in the test are familiar with the expected behaviour
		\item Ensure others in the vicinity of the test are aware of the test and are wearing safety goggles.
		\item Have a safety pilot who is ready to implement the emergency stop at any sign of unexpected behaviour
		\item The safety pilot must call out each command before sending it (except emergency stop, which needs to be done with no delay). These commands include taking off, switching to the offboard (autonomous) mode, and any other commands relevant to the test.
	\end{itemize}
\end{itemize}

\section{Batteries}
Given that all the rollocopters use Lithium ion batteries, procedures for preventing and dealing with battery fires are critical. Hence, the following procedures are in place.

\subsection{Using Batteries}
While using a battery, a battery monitor must be connected and set such that the minimum voltage from each cell is 3.6V, if flying, or 3.8V if running electronics. Note that the discrepancy is due to the slight decrease in voltage when there is a high current drain, such as the propellers. This step is mainly to maintain battery health. If a battery is drained beyond the specified limit, it may cause a fire when next charged.

\subsection{Charging Batteries}
The charging stations are designated areas where the batteries and chargers are kept. This allows for everyone to be aware of where any such issues may arise. When charging a battery, the charger must be in 'Balanced Charge' mode, ensuring that all of the cells are equally charged. In addition, the battery must be kept in a LiPo-safe bag. This is to ensure that, if the battery does explode, the fire will be largely contained by the bag. Finally, the person who connects the battery to the charger is responsible for monitoring it and removing it when fully charged. This is unless the person has explicitly transferred the responsibility to another team member in the lab. No batteries can be left charging unattended. In addition, never charge the batteries on the vehicle. This was brought to the attention of the organisation when RoboSimian caught on fire due to a LiPo battery was charging and suffered.

\subsection{Procedures to Mitigate Consequences}
In the case that one anticipates that a battery might explode (if the battery was used beyond the limit, for example), it must be placed in a LiPo-safe bag and inside a bucket of sand until it can be safely disposed of by the fire department. 

In the case of the RoboSimian fire, a worker attempted to use a fire extinguisher, which did not achieve anything. The fire department was contacted but were unable to stop the fire and had to take the robot out of the lab and allow it to finish burning. The building was evacuated for a few weeks to ensure that all toxic fumes had exited the building.

\section{Checklist Before Leaving}
Before leaving the lab in the evening, the last worker in the lab is required to use the following checklist.

\begin{itemize}
	\item Remove all batteries from the charger and store in a LiPo-safe bag
	\item Remove all battery monitors from all the batteries
	\item Turn off robot transmitters and store in a safe place
	\item Ensure all robots are kept in a safe location and powered off
	\item PPE and tools must be returned to their designated locations
	\item Communal work stations must be cleared of clutter
	\item Switch off all lights and lock the door
\end{itemize}

This aims to eliminate the risk of unmonitored batteries or robots causing difficulty and ensures a smooth start in the lab the next morning.

\section{Field Trips}
Each field trip involves a safety team which creates a plan for the tests to be completed during the trip. By combining this plan with information about the location of the field trip, the safety team can evaluate the safety risks and cover the methods for preventing or managing these situations. All those who intend to be involved in the field trip are then required to attend a briefing to cover the safety protocols. After the field day, there is a debrief meeting in which the safety of the event will be discussed. 
